DiffPlace: A Conditional Diffusion Framework for Simultaneous VLSI Placement Beyond Sequential Paradigms

Chip placement, a critical step in the VLSI physical design flow, directly impacts performance, power, and routability. Traditional chip placement methods, relying on analytical optimization or sequential reinforcement learning (RL), face significant challenges in modern VLSI design, including the inability to consistently satisfy hard placement constraints and the requirement for computationally expensive online training for each new circuit design. Furthermore, existing sequential decision-making paradigms often suffer from compounding errors and extreme wirelength minimization that aggressively compresses modules into dense clusters, leading to severe routing congestion hotspots and failures in downstream design stages. To address these limitations, we introduce DiffPlace, a framework that reformulates chip placement as a conditional denoising diffusion process, enabling transferable policies that generalize to unseen netlists without extensive retraining. Unlike sequential paradigms, DiffPlace simultaneously optimizes all macro positions utilizing a neural backbone equipped with vector-wise message passing to capture geometric dependencies. By prioritizing a more balanced spatial distribution of macros, our framework adopts a routability-first perspective to effectively prevent routing hotspots while maintaining competitive wirelength. To effectively handle the multi-objective nature of placement, we propose a decoupled guidance mechanism: global objectives are optimized via energy-based conditioning, while local physical constraints are actively mitigated through explicit manifold gradient injection during the reverse sampling process. Extensive experiments demonstrate that DiffPlace achieves competitive placement quality while offering superior generalization efficiency compared to state-of-the-art learning-based baselines.

==> sections/IEEE-bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/Le-Trung-Kien.jpg}}]{Le Trung Kien}
received his B.E. in Electronics and Telecommunications from Hanoi University of Science and Technology, Vietnam. Currently, he is a Research Assistant working under the guidance of Dr. Truong-Son Hy at The University of Alabama at Birmingham, United States. His research interests include chip design, hardware acceleration, and time series analysis.
\end{IEEEbiography}
\vspace{5pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/Hy-Truong-Son-333x500.jpg}}]{Dr. Truong Son Hy}
%\begin{IEEEbiographynophoto}{Dr. Hy Truong Son}
is currently a Tenure-Track Assistant Professor in the Department of Computer Science, The University of Alabama at Birmingham, United States. He has earned his Ph.D. in Computer Science from The University of Chicago and his B.Sc. in Computer Science from E\"{o}tv\"{o}s Lor\'{a}nd University. Prior to his current faculty position, he has worked as a lecturer and postdoctoral fellow in the Halıcıoğlu Data Science Institute at the University of California, San Diego; and a tenure-track Assistant Professor in the Department of Mathematics and Computer Science at Indiana State University. His research focuses on graph neural networks, multiresolution matrix factorization, graph wavelets, deep generative models of graphs, group equivariant, and multiscale hierarchical models for scientific applications in the direction of \textbf{AI for Science and Engineering}.
\end{IEEEbiography}

==> sections/abstract.tex <==
% \begin{abstract}
% \label{sec:abstract}
% Chip placement, a critical step in the VLSI physical design flow, directly impacts performance, power, and routability. Traditional methods relying on analytical optimization or reinforcement learning (RL) struggle with hard placement constraints or require computationally expensive online training for each new circuit design. 
% To address these limitations, we introduce DiffPlace, a framework that formulates chip placement as a conditional denoising diffusion process, enabling transferable policies that generalize to unseen netlists without extensive retraining. 
% Unlike sequential wirelength-based decision-making paradigms, \modelname simultaneously optimizes all macro positions utilizing a neural backbone equipped with vector-wise message passing to capture geometric dependencies. By prioritizing a more balanced spatial distribution of macros, our framework effectively prevents the formation of routing hotspots, acknowledging that extreme minimization of wirelength can often lead to congestion-related failures in downstream design stages.
% To effectively handle the multi-objective nature of placement, we propose a decoupled guidance mechanism: global objectives are optimized via energy-based conditioning, while local physical constraints are actively mitigated through explicit manifold gradient injection during the reverse sampling process. Extensive experiments demonstrate that DiffPlace achieves competitive placement quality in terms of wirelength and constraint compliance, while offering superior generalization efficiency compared to state-of-the-art learning-based baselines. We provide a demonstration implementation of the proposed method at: \url{https://github.com/HySonLab/DiffPlace/}.
% \end{abstract}

\begin{abstract}
\label{sec:abstract}
Chip placement, a critical step in the VLSI physical design flow, directly impacts performance, power, and routability. Traditional chip placement methods, relying on analytical optimization or sequential reinforcement learning (RL), face significant challenges in modern VLSI design, including the inability to consistently satisfy hard placement constraints and the requirement for computationally expensive online training for each new circuit design. Furthermore, existing sequential decision-making paradigms often suffer from compounding errors and extreme wirelength minimization that aggressively compresses modules into dense clusters, leading to severe routing congestion hotspots and failures in downstream design stages. To address these limitations, we introduce \modelname, a framework that reformulates chip placement as a conditional denoising diffusion process, enabling transferable policies that generalize to unseen netlists without extensive retraining. Unlike sequential paradigms, \modelname simultaneously optimizes all macro positions utilizing a neural backbone equipped with vector-wise message passing to capture geometric dependencies. By prioritizing a more balanced spatial distribution of macros, our framework adopts a routability-first perspective to effectively prevent routing hotspots while maintaining competitive wirelength. To effectively handle the multi-objective nature of placement, we propose a decoupled guidance mechanism: global objectives are optimized via energy-based conditioning, while local physical constraints are actively mitigated through explicit manifold gradient injection during the reverse sampling process. Extensive experiments demonstrate that \modelname achieves competitive placement quality while offering superior generalization efficiency compared to state-of-the-art learning-based baselines. 

We provide a demonstration implementation of the proposed method at: \url{https://anonymous.4open.science/r/DiffPlace-76F8}.
\end{abstract}
